Conifer Seedling Detection in UAV-Imagery with RGB-Depth Information

Monitoring of reforestation is currently being considerably streamlined through the use of drones and image recognition algorithms, which have already proven to be effective on colour imagery. In addition to colour imagery, elevation data is often also available. The primary aim of this work was to improve the performance of the faster-RCNN object detection algorithm by integrating this height information, which showed itself to notably improve performance. Interestingly, the structure of the network played a key role, with direct addition of the height information as a fourth image channel showing no improvement, while integration after the backbone network and before the region proposal network led to marked improvements. This effect persisted with very long training regimes. Increasing the resolution of this height information also showed little effect.

==> figures/HD_table.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Standard resolution &  High resolution \\
\midrule
Without pretraining &             0.544233 &         0.562725 \\
With pretraining    &             0.601030 &         0.605460 \\
\bottomrule
\end{tabular}


==> figures/main_table.tex <==
\begin{tabular}{lrrrr}
\toprule
Model Name &     Final &     First &   Pre-RPN &   Vanilla \\
\midrule
Without pretraining &  0.286245 &  0.265722 &  0.612378 &  0.289455 \\
With pretraining    &  0.570070 &  0.570959 &  0.704036 &  0.579208 \\
\bottomrule
\end{tabular}

